Linguistic Binding in Diffusion Models: Enhancing Attribute Correspondence through Attention Map Alignment

Text-conditioned image generation models often generate incorrect associations between entities and their visual attributes. This reflects an impaired mapping between linguistic binding of entities and modifiers in the prompt and visual binding of the corresponding elements in the generated image. As one notable example, a query like "a pink sunflower and a yellow flamingo" may incorrectly produce an image of a yellow sunflower and a pink flamingo. To remedy this issue, we propose SynGen, an approach which first syntactically analyses the prompt to identify entities and their modifiers, and then uses a novel loss function that encourages the cross-attention maps to agree with the linguistic binding reflected by the syntax. Specifically, we encourage large overlap between attention maps of entities and their modifiers, and small overlap with other entities and modifier words. The loss is optimized during inference, without retraining or fine-tuning the model. Human evaluation on three datasets, including one new and challenging set, demonstrate significant improvements of SynGen compared with current state of the art methods. This work highlights how making use of sentence structure during inference can efficiently and substantially improve the faithfulness of text-to-image generation.

==> Figures/positive_negative_ablation_main.tex <==
\begin{figure}[t]
  \centering
      \includegraphics[width=0.6\linewidth]{Figures/positive_negative_ablation_main_paper.pdf}
    \caption{\textbf{The impacts of using only one or neither of the loss terms.}
    The absence of a negative loss term leads to semantic leakage (the bird is white) and entity neglect (there is no crown), while the absence of a positive loss term can also lead to semantic leakage (generating a bird and background with white parts), as well as failed attribution binding (generating a crown that is not white).
    }
  \label{fig:positive_negative_ablation_main}
\end{figure}

==> Tables/aae_dataset_human_eval.tex <==
\begin{table}
    \caption{Human Evaluation results on 200 random ABC-6K samples. We report majority vote of 3 raters over 200 HITs (per rater), normalized to 100. \gal{ in the suppl add a short paragrpah that explains how we computed this.}}
   \label{tables:3c_human_eval}
  \centering
  \begin{tabular}{lll}
    \toprule
    Model     & Concept Separation     & Visual Appeal \\
    \midrule
    Syntax        & $\textbf{31.5} \pm 0.15$ & $\textbf{19} \pm 0.07$ \\
    A\&E          & $9 \pm 0.08$ & $6.5 \pm 0.12$ \\
    Structured    & $4 \pm 0.05$  & $3.5 \pm 0.05$ \\
    Standard      & $4 \pm 0.05$  & $9 \pm 0.08$ \\
    No winner & $51.5 \pm 0.18$  & $62 \pm 0.2$ \\
    \bottomrule
  \end{tabular}
\end{table}


==> Tables/abc_6k_200.tex <==
\begin{table}
    \caption{Human Evaluation results on 210 random ABC-6K samples. We report majority vote of 3 raters over 200 HITs (per rater), normalized to 100. \gal{ in the suppl add a short paragrpah that explains how we computed this.}}
   \label{tables:3c_human_eval}
  \centering
  \begin{tabular}{lll}
    \toprule
    Model     & Concept Separation     & Visual Appeal \\
    \midrule
    Syntax        & $\textbf{31.5} \pm 0.15$ & $\textbf{19} \pm 0.07$ \\
    A\&E          & $9 \pm 0.08$ & $6.5 \pm 0.12$ \\
    Structured    & $4 \pm 0.05$  & $3.5 \pm 0.05$ \\
    Standard      & $4 \pm 0.05$  & $9 \pm 0.08$ \\
    No winner & $51.5 \pm 0.18$  & $62 \pm 0.2$ \\
    \bottomrule
  \end{tabular}
\end{table}


==> Tables/ablation_exp.tex <==
\begin{SCtable}
    \scalebox{0.9}{
    \setlength{\tabcolsep}{1pt} %
    \begin{tabular}{llcc}
    \toprule
     Loss & \begin{tabular}[c]{@{}c@{}}Concept\\ Separation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Visual\\ Appeal\end{tabular} \\
    \midrule
    Both losses $\mathcal{L_{Pos}} + \mathcal{L_{Neg}}$& $\textbf{27\%}$ & 22\% \\
    Positive only $\mathcal{L_{Pos}}$& $0\%$ & 11\% \\
    Negative only $\mathcal{L_{Neg}}$& $3\%$ & \textbf{35}\% \\
    Stable Diffusion & $4\%$ & 28\% \\
    No winner & $66\%$ & 4\% \\
    \bottomrule
   \end{tabular}
  }
\label{table:ablation_table}  
\end{SCtable}



==> Tables/complex_concept_conjunction_human_eval_1.tex <==
\begin{table}[h]
    \caption{Human Evaluation results on the Complex Concept Conjunction dataset. We report majority vote of 3 raters over 600 HITs (per rater), normalized to 100. \gal{ in the suppl add a short paragrpah that explains how we computed this.}}
   \label{tables:3c_human_eval}
  \centering
  \begin{tabular}{lrr}
    \toprule
    Model     & Concept Separation     & Visual Appeal \\
    \midrule
    Syntax        & $\textbf{33.5} \pm 0.155$ & $\textbf{20} \pm 0.12$ \\
    A\&E          & $15.5 \pm 0.22$ & $14 \pm 0.1$ \\
    Structured    & $2.5 \pm 0.045$  & $5.5 \pm 0.06$ \\
    Standard      & $1 \pm 0.02$  & $5 \pm 0.06$ \\
    No winner & $47.5 \pm 0.18$  & $55.5 \pm 0.19$ \\
    \bottomrule
  \end{tabular}
\end{table}

